Stability of Topic Modeling via Matrix Factorization

Topic models can provide us with an insight into the underlying latent structure of a large corpus of documents. A range of methods have been proposed in the literature, including probabilistic topic models and techniques based on matrix factorization. However, in both cases, standard implementations rely on stochastic elements in their initialization phase, which can potentially lead to different results being generated on the same corpus when using the same parameter values. This corresponds to the concept of "instability" which has previously been studied in the context of $k$-means clustering. In many applications of topic modeling, this problem of instability is not considered and topic models are treated as being definitive, even though the results may change considerably if the initialization process is altered. In this paper we demonstrate the inherent instability of popular topic modeling approaches, using a number of new measures to assess stability. To address this issue in the context of matrix factorization for topic modeling, we propose the use of ensemble learning strategies. Based on experiments performed on annotated text corpora, we show that a K-Fold ensemble strategy, combining both ensembles and structured initialization, can significantly reduce instability, while simultaneously yielding more accurate topic models.

==> tab-20tp-data.tex <==
%!TEX root = aics2016-ensemble.tex
\begin{table}[!t]
\centering
\caption{Number of tweets, unique user accounts, and user documents for each topic in the \emph{20-topics} dataset.}
\label{tab:20tp-data}
\begin{tabular}{|p{2.6cm}|P{2cm}|P{2cm}|P{2.9cm}|}
\hline
\textbf{Category} & \textbf{Tweets} & \textbf{Users} & \textbf{User Documents} \\  \hline
Aviation          & 186,641                    & 57                       & 2,440                              \\ 
Basketball        & 245,359                    & 61                       & 1,467                              \\ 
Business          & 223,148                    & 70                       & 1,876                              \\ 
Energy            & 125,130                    & 40                       & 1,621                              \\ 
Fashion           & 159,819                    & 40                       & 1,227                              \\ 
Food              & 159,615                    & 45                       & 1,775                              \\ 
Football          & 359,393                    & 89                       & 1,524                              \\ 
Formula One       & 143,197                    & 42                       & 1,757                              \\ 
Health            & 209,941                    & 60                       & 2,542                              \\ 
Irish Politics    & 170,000                    & 50                       & 2,318                              \\ 
Movies            & 139,337                    & 38                       & 1,395                              \\ 
Music             & 208,838                    & 56                       & 1,539                              \\ 
NFL               & 255,554                    & 80                       & 1,388                              \\ 
Rugby             & 265,123                    & 76                       & 2,264                              \\ 
Space             & 127,280                    & 51                       & 2,157                              \\ 
Tech              & 250,486                    & 66                       & 1,947                              \\ 
Tennis            & 139,067                    & 41                       & 1,427                              \\ 
UK Politics       & 245,651                    & 77                       & 3,182                              \\ 
US Politics       & 332,766                    & 103                      & 4,503                              \\ 
Weather           & 224,037                    & 65                       & 2,373                              \\ \hline 
\end{tabular}
\end{table}


==> tab-ensemble-topics.tex <==
%!TEX root = aics2016-ensemble.tex
\begin{table}[!t]
\centering
\caption{Topic descriptors for 20 topics generated by applying ensemble topic modeling to the \emph{20-topics} corpus, using tweets from 1,200 core users. The most similar ground truth category for each topic is also listed.}
\label{tab:topics}
\begin{tabular}{|p{1.9cm}|p{9.5cm}|}
\hline
\textbf{Category} & \textbf{Top 10 Terms}                                                                          \\ \hline
Energy 1       & fracking, shale, gas, energy, natgas, natural, naturalgas, pa, epa, emissions         \\ 
US Politics    & gopdebate, president, gop, obama, senate, clinton, bill, hillary, trump, congress     \\ 
Rugby          & rugby, rwc2015, england, cup, wales, ireland, world, try, match, rbs6nations          \\ 
NFL            & game, nfl, season, win, patriots, team, league, football, tonight, goal               \\ 
Tech 1         & apple, watch, applewatch, google, app, music, tv, ios, facebook, macbook              \\ 
UK Politics    & labour, ge16, people, tories, vote, tory, party, government, nhs, support             \\ 
Basketball     & bulls, rose, butler, hoiberg, gasol, nba, game, noah, jimmy, pau                      \\ 
Weather        & rain, snow, weather, forecast, showers, storm, tornado, severe, dry, winds            \\ 
Business       & china, stocks, market, fed, markets, stock, growth, tech, uk, ftse                    \\ 
Health         & health, cancer, study, risk, patients, care, diabetes, zika, drug, disease            \\ 
Music          & album, music, video, listen, song, track, remix, tour, premiere, check                \\ 
Aviation       & avgeek, aviation, boeing, flight, airlines, air, aircraft, airbus, airport, paxex     \\ 
Tech 2         & iphone, ios, ipad, mac, apple, app, os, apps, beta, plus                              \\ 
Fashion        & fashion, daily, nyfw, stories, style, collection, dress, wear, beauty, show           \\ 
Food           & recipes, recipe, food, chicken, best, dinner, delicious, chocolate, chef, restaurant  \\ 
Formula One      & f1, race, ferrari, hamilton, mclaren, mercedes, renault, rosberg, gp, bull            \\ 
Movies         & film, review, movie, trailer, star, wars, movies, films, awakens, oscars              \\ 
Tennis         & tennis, atp, murray, djokovic, federer, serena, nadal, wimbledon, ausopen, wta        \\ 
Space          & space, yearinspace, pluto, earth, nasa, mars, mission, launch, journeytomars, science \\ 
Energy 2       & oil, energy, gas, crude, prices, opec, offshore, production, exports, oilandgas       \\  \hline
\end{tabular}
\end{table}

==> tab-example-nmf.tex <==
\begin{table}[!t]
\begin{center}
\caption{Top-ranked terms for a set of five related topics, as generated by applying randomly-initialized NMF to a corpus of news articles.}
\vskip 0.5em
\begin{scriptsize}
\begin{tabular}{c|p{3.15in}}
\hline
\textbf{\#} & \textbf{Top 10 Terms}                                                                      \\ \hline
1                     & cent, ireland, tax, bank, bailout, government, euro, economy, noonan, finance     \\ 
2                     & cent, tax, rate, economy, growth, budget, unemployment, prices, quarter, economic \\ 
3                     & cent, tax, ireland, bank, bailout, government, euro, economy, growth, finance     \\ 
4                     & cent, ireland, tax, bank, bailout, government, euro, economy, growth, noonan      \\ 
5                     & cent, tax, rate, economy, growth, budget, unemployment, prices, quarter, property \\ \hline
\end{tabular}
\end{scriptsize}
\label{tab:nmf}
\end{center}
\end{table}
